SCExAO/CHARIS Spectroscopic Characterization of Cloudy L/T Transition Companion Brown Dwarf HIP 93398 B

Brown dwarfs with measured dynamical masses and spectra from direct imaging are benchmarks that anchor substellar atmosphere cooling and evolution models. We present Subaru SCExAO/CHARIS infrared spectroscopy of HIP 93398 B, a brown dwarf companion recently discovered by Li et al. 2023 as part of an informed survey using the Hipparcos-Gaia Catalog of Accelerations. This object was previously classified as a T6 dwarf based on its luminosity, with its independently-derived age and dynamical mass in tension with existing models of brown dwarf evolution. Spectral typing via empirical standard spectra, temperatures derived by fitting substellar atmosphere models, and J-H, J-K and H-L' colors all suggest that this object has a substantially higher temperature and luminosity, consistent with classification as a late-L dwarf near the L/T transition (T = 1200$^{+140}_{-119}$ K) with moderate to thick clouds possibly present in its atmosphere. When compared with the latest generation of evolution models that account for clouds with our revised luminosity and temperature for the object, the tension between the model-independent mass/age and model predictions is resolved.

==> table1_orig.tex <==
\begin{table}
\resizebox{\linewidth}{!}{%
\begin{tabular}{|lcc|}
\hline
\multicolumn{1}{|c|}{\textbf{Property}} & \multicolumn{1}{c|}{\textbf{Value}} & \textbf{References} \\ \hline
\multicolumn{3}{|c|}{Host Star (A)} \\ \hline
\multicolumn{1}{|l|}{$\varpi$ (mas)} & \multicolumn{1}{c|}{27.033$\pm$0.018} & 1 \\ \hline
\multicolumn{1}{|l|}{Distance (pc)} & \multicolumn{1}{c|}{36.99$\pm$0.03} & 1 \\ \hline
\multicolumn{1}{|l|}{SpT} & \multicolumn{1}{c|}{K3.5V} & 2,3 \\ \hline
\multicolumn{1}{|l|}{Mass (M$_\odot$)} & \multicolumn{1}{c|}{0.72$\pm$0.02} & 4,5 \\ \hline
\multicolumn{1}{|l|}{Age (Gyr)} & \multicolumn{1}{c|}{3.59$^{+0.87}_{-1.15}$} & 12 \\ \hline
\multicolumn{1}{|l|}{T$_{eff}$ (K)} & \multicolumn{1}{c|}{4727$\pm$104} & 6 \\ \hline
\multicolumn{1}{|l|}{[Fe/H] (dex)} & \multicolumn{1}{c|}{-0.15$\pm$0.07} & 7 \\ \hline
\multicolumn{1}{|l|}{log($R'_{HK}$) (dex)} & \multicolumn{1}{c|}{-4.85} & 8 \\ \hline
\multicolumn{1}{|l|}{$R'_X$ (dex)} & \multicolumn{1}{c|}{$<$-4.28} & 9 \\ \hline
\multicolumn{1}{|l|}{log$g$ (dex)} & \multicolumn{1}{c|}{4.64$^{+0.0846}_{-1.203}$} & 14 \\ \hline
\multicolumn{1}{|l|}{\textit{Gaia} RUWE} & \multicolumn{1}{c|}{1.019} & 1 \\ \hline
\multicolumn{1}{|l|}{Luminosity (L$_\odot$)} & \multicolumn{1}{c|}{0.208$\pm$0.007} & 12 \\ \hline
\multicolumn{1}{|l|}{\textit{Gaia} G (mag)} & \multicolumn{1}{c|}{9.374$\pm$0.003} & 1 \\ \hline
\multicolumn{1}{|l|}{$B_T$ (mag)} & \multicolumn{1}{c|}{11.195$\pm$0.066} & 10 \\ \hline
\multicolumn{1}{|l|}{$V_T$ (mag)} & \multicolumn{1}{c|}{9.923$\pm$0.035} & 10 \\ \hline
\multicolumn{1}{|l|}{$J$ (mag)} & \multicolumn{1}{c|}{7.804$\pm$0.027} & 11 \\ \hline
\multicolumn{1}{|l|}{$H$ (mag)} & \multicolumn{1}{c|}{7.313$\pm$0.033} & 11 \\ \hline
\multicolumn{1}{|l|}{$K_s$ (mag)} & \multicolumn{1}{c|}{7.175$\pm$0.020} & 11 \\ \hline
\multicolumn{3}{|c|}{Companion (B)} \\ \hline
\multicolumn{1}{|l|}{SpT} & \multicolumn{1}{c|}{L9.0} & 13 \\ \hline
\multicolumn{1}{|l|}{Mass ($M_{\textup{Jup}}$)} & \multicolumn{1}{c|}{65.9$^{+2.0}_{-1.7}$} & 12 \\ \hline
%\multicolumn{1}{|l|}{$J$ apparent (mag)} & \multicolumn{1}{c|}{11.07$\pm$0.93} & 13 \\ \hline
%\multicolumn{1}{|l|}{$J$ absolute (mag)} & \multicolumn{1}{c|}{8.226$\pm$0.93} & 13 \\ \hline
\multicolumn{1}{|l|}{$H$ apparent (mag)} & \multicolumn{1}{c|}{16.51$\pm$0.07} & 13 \\ \hline
\multicolumn{1}{|l|}{$H$ absolute (mag)} & \multicolumn{1}{c|}{13.67$\pm$0.07} & 13 \\ \hline
\multicolumn{1}{|l|}{$J$ apparent (mag)} & \multicolumn{1}{c|}{17.54$\pm$0.33} & 13 \\ \hline
\multicolumn{1}{|l|}{$J$ absolute (mag)} & \multicolumn{1}{c|}{14.70$\pm$0.33} & 13 \\ \hline
\multicolumn{1}{|l|}{$L'$ apparent (mag)} & \multicolumn{1}{c|}{16.31$\pm$0.07} & 12 \\ \hline
\multicolumn{1}{|l|}{$L'$ absolute (mag)} & \multicolumn{1}{c|}{13.47$\pm$0.07} & 12 \\ \hline
\multicolumn{1}{|l|}{log($L_{\textup{bol}}/L_\odot)$} & \multicolumn{1}{c|}{-5.26$\pm$0.07} & 12 \\ \hline
\multicolumn{1}{|l|}{Semimajor axis (AU)} & \multicolumn{1}{c|}{11.05$^{+0.64}_{-0.56}$} & 12 \\ \hline
\multicolumn{1}{|l|}{Inclination ($^\circ$)} & \multicolumn{1}{c|}{48.9$^{+3.4}_{-3.7}$} & 12 \\ \hline
\multicolumn{1}{|l|}{Period (yr)} & \multicolumn{1}{c|}{40.6$^{+3.9}_{-3.5}$} & 12 \\ \hline
\multicolumn{1}{|l|}{Eccentricity} & \multicolumn{1}{c|}{0.496$^{+0.022}_{-0.020}$} & 12 \\ \hline
\multicolumn{1}{|l|}{Temperature (K)} & \multicolumn{1}{c|}{1300$^{+81}_{-150}$} & 13 \\ \hline
\end{tabular}%
}
\caption{Table summarizing the previously known and new properties of the HD 176535 AB system. References abbreviated as (1) \citet{GaiaCollaboration2020A&A}; (2) \citet{Gray2006AJ}; (3) \citet{Bourges2014ASPC}; (4) \citet{Reiners2020ApJS}; (5) \citet{DelgadoMena2019A&A}; (6) \citet{Sousa2011A&A}; (7) \citet{Gaspar2016ApJ}; (8) \citet{Pace2013A&A}; (9) \citet{Voges1999ICRC}; (10) \citet{Hog2000eaa}; (11) \citet{Cutri2003yCat}; (12) \citet{Li2023MNRAS}; (13) this work; and (14) \citet{Stassun2019yCat}.}
\label{tab:sysprops}
\end{table}
